Efficient Nearest-Neighbor Search for Dynamical Systems with Nonholonomic Constraints

Nearest-neighbor search dominates the asymptotic complexity of sampling-based motion planning algorithms and is often addressed with k-d tree data structures. While it is generally believed that the expected complexity of nearest-neighbor queries is $O(log(N))$ in the size of the tree, this paper reveals that when a classic k-d tree approach is used with sub-Riemannian metrics, the expected query complexity is in fact $\Theta(N^p \log(N))$ for a number $p \in [0, 1)$ determined by the degree of nonholonomy of the system. These metrics arise naturally in nonholonomic mechanical systems, including classic wheeled robot models. To address this negative result, we propose novel k-d tree build and query strategies tailored to sub-Riemannian metrics and demonstrate significant improvements in the running time of nearest-neighbor search queries.

==> macros.tex <==
% set pdf figure transparency problems
\pdfpageattr {/Group << /S /Transparency /I true /CS /DeviceRGB>>}

\usepackage{amsmath, amsthm, amssymb, bm, enumerate, url, setspace}
\usepackage[usenames,dvipsnames,svgnames,table]{xcolor}
\usepackage[bookmarks=true]{hyperref}
\hypersetup{
colorlinks=true, linkcolor=blue, citecolor=ForestGreen, filecolor=magenta, urlcolor=blue,
}
\usepackage[numbers, sort&compress]{natbib}

\setlength{\marginparwidth}{0.8in}
\newcommand{\vvcolor}{\color{cyan}}
\newcommand{\vv}[2]{{\vvcolor #1}\marginpar{\tiny\noindent{\raggedright{\vvcolor [VV] #2 \par}}}}
\newcommand{\dycolor}{\color{magenta}}
\newcommand{\dy}[2]{{\dycolor #1}\marginpar{\tiny\noindent{\raggedright{\dycolor [DY] #2 \par}}}}
\newcommand{\todo}[1]{{\color{gray}#1}\marginpar{\tiny\noindent{\raggedright{\color{ForestGreen}[MILD TODO]}}}}
